On the Cost of Evolving Task Specialization in Multi-Robot Systems

Task specialization can lead to simpler robot behaviors and higher efficiency in multi-robot systems. Previous works have shown the emergence of task specialization during evolutionary optimization, focusing on feasibility rather than costs. In this study, we take first steps toward a cost-benefit analysis of task specialization in robot swarms using a foraging scenario. We evolve artificial neural networks as generalist behaviors for the entire task and as task-specialist behaviors for subtasks within a limited evaluation budget. We show that generalist behaviors can be successfully optimized while the evolved task-specialist controllers fail to cooperate efficiently, resulting in worse performance than the generalists. Consequently, task specialization does not necessarily improve efficiency when optimization budget is limited.

==> conference_instructions.tex <==
\section{Conference-specific instructions}

\subsection{Important Dates}
\begin{itemize}
    \item Submission deadline: November 10, 2025
    \item Notification of acceptance: January 30, 2026
    \item Camera ready copy: February 13, 2026
    \item Conference: June 8-10, 2026
\end{itemize}

\subsection{Submission}
Submissions may be a maximum of 11 pages, excluding references, when typeset in the Springer Lecture Notes in Computer Science (LNCS) LaTeX template. Submissions should be a minimum of 7 full pages.

This strict page limit includes figures, tables, and all supplementary sections (e.g., Acknowledgements). The only exclusion from the page limit is the reference list, which should be of any length suitable to adequately position the paper with respect to the state of the art.

Papers should be prepared in English, in the Springer LNCS LaTeX style, using the default font and font size. Authors should consult Springer’s authors’ guidelines and use their proceedings template for LaTeX, for the preparation of their papers. Please download the Proceedings (LNCS) LaTex template package (zip, 318 kB) and authors' guidelines (pdf, 244 kB) directly from the Springer website.

Submissions that do not respect these guidelines will not be considered.

The initial submission must be in PDF format.

Please note that in the camera-ready phase, authors of accepted papers will need to submit both a compiled PDF and all source files (including LaTeX files and figures).

The camera-ready phase will have more detailed formatting requirements than the initial submission phase.

\subsection{Submission process}

Submitted papers will be peer-reviewed on the basis of technical quality, relevance, significance, and clarity. If a submission is not accepted as a full length paper, it may still be accepted either as a short paper or as an extended abstract. In such cases, authors will be asked to reduce the length of the submission accordingly. Authors of all accepted papers will be asked to execute revisions, based on the reviewers’ comments.
Use of large language models
We ask all authors and reviewers to adhere to the Springer Nature policy regarding the use of AI: Springer: Artificial Intelligence (AI) 
